Task Abstention for Large Language Models in Code Generation

Large language models (LLMs) have revolutionized automated code generation. One serious concern, however, is the so-called ``hallucination'', i.e., LLMs may generate seemingly plausible but functionally incorrect code. In this paper, we study the task abstention problem, i.e., determining whether a given LLM should abstain from performing a specific code generation task to avoid likely hallucination. Our approach features a calibrated abstention rule, grounded in the principles of multiple hypothesis testing. The rule assesses generation consistency through code execution outcomes, allowing it to handle syntactic diversity of semantically equivalent code without reliance on oracle test cases or external databases. We prove that our approach provides a rigorous, distribution-free theoretical guarantee on its abstention decisions. We evaluate our method on benchmark datasets using several open-source code LLMs. Results show that our method allows generative models to more accurately and efficiently identify and abstain from tasks that induce hallucination compared to existing techniques, providing a reliable mechanism for safer and more robust code generation.

==> src/effi.tex <==
% \input{tables/transfer_result}

\section{Implementation Details of Efficient Sampling}\label{appd:effi}
In the testing phase, the standard procedure requires generating a fixed, often large number of samples (e.g., 256) to ensure statistical robustness. However, generating such a volume of code and test cases for every query is computationally expensive and increases latency.

We propose an efficient sampling strategy motivated by the empirical observation that for solvable tasks, semantic consistency among code samples typically emerges after only a few generations. Conversely, tasks that induce hallucination tend to remain inconsistent even as the sample size increases. Based on this insight, we implement an iterative, batched sampling mechanism, formally presented in Alg.~\ref{alg:EffSampling}. The procedure operates as follows.

\noindent \textbf{Initialization.} The process begins by initializing empty sets for code samples  and test cases , along with a counter for the current number of samples.

\noindent \textbf{Iterative Generation.} The algorithm enters a loop that continues as long as the current sample count is below the maximum budget . In each iteration, instead of generating the full quota, the model generates a small batch of size  (e.g., 8 samples). These new outputs are immediately merged into the cumulative sets  and .

\noindent \textbf{Incremental Evaluation.} Once the cumulative sets are updated, the core inference logic (as described in Alg.~\ref{alg:UnifiedFilter} of the main text) is applied to the current  and . This step checks if the current pool of samples already satisfies the admission criteria defined by the thresholds .

\noindent \textbf{Early Termination and Fallback.} If the evaluation returns an \textit{Admit} decision—meaning a sufficiently consistent cluster has emerged or entropy has dropped below the threshold—the loop terminates immediately, returning the result. This allows solvable tasks to exit the loop early, saving significant computational resources. If the maximum budget  is exhausted without meeting the admission criteria, the algorithm concludes that the model cannot solve the task consistently and returns \textit{Abstain}.

\begin{algorithm}[h]\caption{Efficient Sampling}
\label{alg:EffSampling}
\begin{algorithmic}[1]\Require LLM $\mathcal{M}$; task prompt $x$; batch size $n_{batch}$; max budget $N_{max}$; calibrated thresholds $\pmb{\lambda}$
\Ensure Abstention decision 
\Procedure{Effi}{$\mathcal{M}, x, n_{batch}, N_{max}, \pmb{\lambda}$}\State $Y_{total} \gets \emptyset$\State $T_{total} \gets \emptyset$\State $n_{curr} \gets 0$\While{$n_{curr} < N_{max}$}
    \State $Y_{batch}, T_{batch} \gets \text{\small Generate}(\mathcal{M}, n_{batch})$
    
    \State $Y_{total} \gets Y_{total} \cup Y_{batch}$
    \State $T_{total} \gets T_{total} \cup T_{batch}$
    \State $n_{curr} \gets n_{curr} + n_{batch}$
    

    \State $res \gets \text{\small CodeRefuser}(\mathcal{M}, x, n_{curr}, \pmb{\lambda})$
    
    \If{$res$ is \textit{Admit}}
        \State \Return \textit{Admit}
    \EndIf
\EndWhile

\State \Return \textit{Abstain}
\EndProcedure\end{algorithmic}\end{algorithm}


% We evaluate the trade-off between sampling cost (i.e., the number of generated code samples and test cases) and abstention accuracy for \name. The experiment is conducted on the HumanEval benchmark using DeepSeek-Coder-33B (DSCoder) and Qwen2.5-Coder-32B (QwenCoder) with parameters set to $\alpha = 0.2, \delta = 0.1$ and $k = 3$.

% To ensure a fair comparison, we first perform a thorough calibration (generating 256 code samples and 256 test cases) to obtain the valid threshold set $\Lambda_{valid}$. For the testing phase, we select the specific threshold that yielded the lowest abstention rate on the calibration set. We then compare the following two approaches:
% \begin{itemize}[leftmargin=*]
%     \item Full sampling (Full), which generates the full budget of 256 code samples and 256 test cases to make the abstention decision.
%     \item Efficient sampling (Effi), which uses our iterative, batched sampling strategy as described in Alg.\ref{alg:EffSampling}, with the maximum sample count up to 256.
% \end{itemize}

% We compare their precision and the average required number of samples in Table~\ref{tab:effi}. The result shows that our method achieves a substantial reduction in the number of required samples while incurring a negligible loss in precision. 

% \input{tables/effi_res}

==> src/limit.tex <==


\section{Limit} \label{sect:threat}

In this section, we identify and discuss several potential threats to the validity of our study and the steps taken to mitigate them.

%\smallskip
\noindent{\bf Generalization to Out-of-Distribution Tasks.}  Our theoretical guarantee relies on the assumption that the calibration and test data are independent and identically distributed. However, in real-world scenarios, the problem a system encounters may differ from those it sees during calibration. This potential distribution shift could introduce bias and weaken the risk control guarantees in practice.
To mitigate this threat, we have conducted experiments using MBPP as calibration data and HumanEval as test data, and the results show that there was no significant decline in performance.

\smallskip
\noindent{\bf Applicability to Non-Deterministic Systems.} The core of our approach--both the score functions and the STDF mechanism--assumes that all tasks have deterministic solutions.  %where a given input always produces a unique output. 
The assumption may not hold for complex, interactive software systems, which may exhibit nondeterminism. As our method relies on clustering identical outputs, its applicability is currently limited to deterministic problem domains.

\smallskip
\noindent{\bf Evaluation Limited to a Single Programming Language.} Current experiments are conducted in Python, a language where modern LLMs have demonstrated strong performance~\cite{huang2024effibench, twist2025llms}. However, many real-world systems are built using other languages such as Java or C, which may have different characteristics % and failure modes 
(e.g., pointer and memory management in C). The effectiveness of our method %remains effective 
in these programming languages %in an open question that 
requires further evaluation. 


==> tables/effi_res.tex <==
\begin{table}[t]
\centering
\caption{The cost-effectiveness of our efficient sampling strategy. Significantly fewer code samples and test cases are needed to keep close precision.}
\vspace{-2mm}
\label{tab:effi}
\begin{tabular}{l | c c }
\toprule
 & \textbf{Prec.} & \textbf{\# Avg Samples} \\
 \midrule

 DSCoder (Full) & 0.61  & 256   \\
 DSCoder (Effi)  & 0.60 & 49.97 \\
 \midrule
 QwenCoder (Full)  &  0.38 & 256  \\
 QwenCoder (Effi) & 0.36 & 47 \\

\bottomrule
\end{tabular}
\end{table}

==> tables/table1.tex <==
\begin{table*}[htbp]
\centering
\caption{Task abstention results on HumanEval. Our approaches (i.e., `SE+STDF' and `CR+STDF') generally outperform the competitors.}
\label{tab:abstentionHE}
\begin{tabularx}{\textwidth}{l | *{8}{C}}
\toprule
 %& \multicolumn{8}{c}{\textbf{HumanEval}} \\
 %\cmidrule(lr){1-9}
 \multirow{2}{*}{\diagbox[trim=l]{Config}{Model}} 
 & \multicolumn{2}{c}{DeepSeek-Coder} & \multicolumn{2}{c}{Qwen2.5-Coder} & \multicolumn{2}{c}{CodeLlama} & \multicolumn{2}{c}{WizardCoder} \\
 & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} \\
 \midrule

 % data
 Execution  & 39.28 &  55.27  &  24.29  &  38.23  & 72.15 &  83.82  &  35.46  &  51.55 \\
 \midrule
 %-----------------------------------------------------------%
 PPL   &  36.41  &  53.39  & 22.22 &  21.43 &  72.29  &  81.67  &  40.90  &  37.11 \\
 \midrule
 %-----------------------------------------------------------%
 NLI  & 49.25 & 52.38 &  17.68  &  30.05  &  77.92 &  62.82  &  31.70  &  48.15 \\
 \midrule
 %-----------------------------------------------------------%
 CLM  &  36.41  &  53.39  &  22.22  & 21.42  &  71.27  &  64.42  & 37.71  &  51.49 \\
 \midrule
 %-----------------------------------------------------------%
 SE   &  61.19  &  65.07  & 38.23  &  41.67  & 85.95  &  88.51  & 52.63  & 62.01 \\
 \midrule
 %-----------------------------------------------------------%
 CR   & 0.6052  &  0.6814  & 0.4444  &  0.4923  & 0.8947 &  0.8947  &  0.4799  & 0.5600 \\
 \midrule
 %-----------------------------------------------------------%
 SE + STDF   & 0.6363   &  0.6667  &  0.4736  &  0.5091  &  \SOTA{0.9167}  &  0.8919  &   \SOTA{0.6271} &  \SOTA{0.6667} \\
 \midrule
 %-----------------------------------------------------------%
 CR + STDF   & \SOTA{0.7200}  &  \SOTA{0.6992}  &  \SOTA{0.7333} &  \SOTA{0.5385}  & \SOTA{0.9167}  & \SOTA{0.9170}  & 0.6140  & 0.6614 \\
 \bottomrule
\end{tabularx}
\end{table*}

==> tables/table2.tex <==
\begin{table*}[htbp]
\centering
\caption{Task abstention results on MBPP. Our approaches (i.e., `SE+STDF' and `CR+STDF') generally outperform the competitors.}
\label{tab:abstentionMBPP}
\begin{tabularx}{\textwidth}{l | *{8}{C}}
\toprule
% & \multicolumn{8}{c}{\textbf{MBPP}} \\
 %\cmidrule(lr){1-9}
 \multirow{2}{*}{\diagbox[width=7em, trim=l]{Config}{Model}} 
 & \multicolumn{2}{c}{DeepSeek-Coder-33B} & \multicolumn{2}{c}{Qwen2.5-Coder-32B} & \multicolumn{2}{c}{CodeLlama-7B} & \multicolumn{2}{c}{WizardCoder-33B} \\
 & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} \\
 \midrule

 % data
 Execution  &  0.4131  &  0.5742  &  0.3150  &  0.4611  & 0.5835 &  0.7301 & 0.3608   & 0.5175 \\
 \midrule
 %-----------------------------------------------------------%
 PPL   & 0.3716  & 0.5111  &  0.3928 &  0.3455  & 0.7124 & 0.5547  & 0.3846  & 0.3433 \\
 \midrule
 %-----------------------------------------------------------%
 NLI   & 0.3940 &  0.4988 & 0.3050  & 0.3961  & 0.6795 & 0.5829  & 0.3313  &  0.3698 \\
 \midrule
 %-----------------------------------------------------------%
 CLM  & 0.3632  &  0.5328  & 0.3160 &  0.4425  &  0.5660 & 0.7228  & 0.3510  & 0.5000 \\
 \midrule
 %-----------------------------------------------------------%
 SE   &  0.6470  &  0.6461  & 0.4074   &  0.4565  &  0.7177  &  0.7902  &  0.6016  &  0.6126 \\
 \midrule
 %-----------------------------------------------------------%
 CR   &  0.6199  &  0.6628  &  0.4000  &  0.4558  &  0.6724  &  0.6567  &  0.6299  & 0.6250 \\
 \midrule
 %-----------------------------------------------------------%
 SE + STDF   &  \SOTA{0.7265}  & \SOTA{0.7288} &  0.4841  &  \SOTA{0.5284}  &  0.7270  &  0.7669  &  0.6026  & \SOTA{0.6470} \\
 \midrule
 %-----------------------------------------------------------%
 CR + STDF   &  0.6643  &  0.6648  & \SOTA{0.4894}  & 0.4744   &  \SOTA{0.7940}  &  \SOTA{0.7969}  &  \SOTA{0.6923}  & 0.6307 \\
 \bottomrule
\end{tabularx}
\end{table*}

==> tables/transfer_result.tex <==
\begin{table*}[htbp]
\centering
\caption{Task abstention results when the calibration is conducted on MBPP and the testing is conducted on HumanEval. Compared to Table~\ref{tab:abstention_main}, our approaches achieve close performance in most cases.} %remain the top-performing approaches, despite a drop in performance for Qwen2.5-Coder-32B model.}
\label{tab:noniid}
\begin{tabularx}{\textwidth}{l | *{8}{>{\centering\arraybackslash}X}}
\toprule
 \multirow{2}{*}{\diagbox[width=6em, trim=l]{Config}{Model}} 
 & \multicolumn{2}{c}{DeepSeek-Coder} & \multicolumn{2}{c}{Qwen2.5-Coder} & \multicolumn{2}{c}{CodeLlama} & \multicolumn{2}{c}{WizardCoder} \\
 & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} & \textbf{P} & \textbf{F1} \\
 \midrule

 % data
 %-----------------------------------------------------------%
 SE   &  60.27  &  62.11  & 32.65   &  41.50  &  76.03 &  78.63  &  60.00  &  58.99 \\
 \midrule
 %-----------------------------------------------------------%
 CR   &  63.01  &  65.08  &  32.65  &  37.68  &  79.79  &  79.48  &  57.41  & 56.88 \\
 \midrule
 %-----------------------------------------------------------%
 SE + STDF   &  \SOTA{71.11}  & \SOTA{70.00} &  39.39  &  \SOTA{50.00}  &  80.28  &  77.27  &  68.42  & 59.65 \\
 \midrule
 %-----------------------------------------------------------%
 CR + STDF   &  66.67  &  66.67  & \SOTA{40.63}  & 40.00   &  \SOTA{91.51}  &  \SOTA{91.23}  &  \SOTA{72.10}  & \SOTA{62.39} \\
 \bottomrule
\end{tabularx}
\end{table*}
